Every Dataset Counts: Scaling up Monocular 3D Object Detection with Joint Datasets Training

Monocular 3D object detection plays a crucial role in autonomous driving. However, existing monocular 3D detection algorithms depend on 3D labels derived from LiDAR measurements, which are costly to acquire for new datasets and challenging to deploy in novel environments. Specifically, this study investigates the pipeline for training a monocular 3D object detection model on a diverse collection of 3D and 2D datasets. The proposed framework comprises three components: (1) a robust monocular 3D model capable of functioning across various camera settings, (2) a selective-training strategy to accommodate datasets with differing class annotations, and (3) a pseudo 3D training approach using 2D labels to enhance detection performance in scenes containing only 2D labels. With this framework, we could train models on a joint set of various open 3D/2D datasets to obtain models with significantly stronger generalization capability and enhanced performance on new dataset with only 2D labels. We conduct extensive experiments on KITTI/nuScenes/ONCE/Cityscapes/BDD100K datasets to demonstrate the scaling ability of the proposed method.

==> secs/image_infer.tex <==
\begin{figure*}
    \centering
    \includegraphics[{width=0.8\textwidth}]{secs/monodepth_infer-crop.pdf}
    \caption{Online inference pipeline of FSNet. Dense full-scale Depth $d_0$ is first predicted from the trained network.  The prediction will be merged with sparse VO points $d_{vo}$ to produce accurate final prediction. The 3D SLIC algorithm is used to segment the image and limit the scale of the post-optimization problem. Only processes within the yellow frame needs to be trained in the training phase.
    }
    \label{fig:monodepth_infer}
\end{figure*}

==> secs/image_init.tex <==
%\begin{figure}
%    \centering
%    \includegraphics[{width=0.35\textwidth}]{secs/monodepth_init_range-crop.pdf}
%    \caption{Using the trained model as the reference, we demonstrate the area with reconstruction error less than 1 pixel. when the initial depth is 15 meters (upper) and 100 meters (lower). These fraction of pixels produce correct gradients at initialization.
    }
%    \label{fig:monodepth_init}
%\end{figure}

==> secs/image_struct.tex <==
\begin{figure*}
    \centering
    \includegraphics[{width=0.8\textwidth}]{secs/monodepth_struct_flow-crop.pdf}
    \caption{The training process of FSNet. Both the teacher network $\Theta_{teacher}$ and the student network $\Theta_{student}$ utilize a U-Net structure with a ResNet-18 backbone.
    $\Theta_{teacher}$ is fully-pretrained using only the photometric loss and is frozen during the training of the student network. $\Theta_{student}$ is trained with a summation of photometric loss and distillation loss. To form the photometric loss, we calculate the optical flow between two frames and use it to compute an extra mask to block error gradients from dynamic objects.
    }
    \label{fig:monodepth_struct}
\end{figure*}

==> secs/sec-0-introduction.tex <==


\section{Introduction}
\label{section:Introduction}






% The pursuit of a comprehensive 3D understanding of dynamic environments stands as a cornerstone in the fields of robotics, autonomous driving, and augmented reality. Contemporary 3D detection algorithms leveraging LiDAR point clouds have shown remarkable performance, owing to the enhanced accuracy and density of these point clouds \cite{Yun2018Focal}. Nevertheless, when contrasted with LiDAR, cameras are found to be cost-effective, power-efficient, and offer greater flexibility in installation. This has led to their widespread use in robots and autonomous vehicles, consequently making 3D detection via single cameras an increasingly compelling area of research within robotics and computer vision.

Precise 3D understanding of the surrounding environment is the cornerstone of fields such as robotics and autonomous driving. In recent years, 3D detection algorithms using LiDAR point clouds have demonstrated outstanding performance, attributed to the precise ranging capabilities of LiDAR \cite{Yun2018Focal}. However, LiDAR is costly and not conducive to large-scale practical applications. In comparison to LiDAR, cameras offer advantages such as low cost, energy efficiency, rich color information, and compact size, providing greater flexibility in installation. These advantages have led to their widespread use in the fields of robotics and autonomous driving, making 3D detection using monocular cameras an increasingly promising research area in robotics and computer vision.

% Over the last few years, monocular 3D object detection \cite{ma20233d} has experienced a significant evolution. Models employing Bird-Eye-View (BEV) representation have notably amplified potential in settings involving multi-sensor fusion, frequently encountered in autonomous driving scenarios. However, models utilizing front-view representation, the inherent representation of camera images, are not only faster but also simpler to deploy.

In recent years, there has been a notable advancement in monocular 3D object detection \cite{ma20233d}. Models utilizing Bird's Eye View (BEV) representation have shown increased effectiveness in scenarios requiring multi-sensor fusion, commonly found in autonomous driving applications. On the other hand, models using front-view representation, which is the natural representation of camera images, are not only quicker but also easier to implement.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{secs/pictures/cover_figure229b.png}
    \captionsetup{font={footnotesize}}
    \captionsetup{justification=justified} % 设置 caption 文字两端对齐
    \vspace{-18pt}
    \caption{Our method mainly consists of three parts. The first part is the camera parameter adaptation module, which handles different camera parameters to mitigate their impact. The second part is multi-dataset joint training, where we pre-train the model using as many datasets as possible to enhance its feature extraction capability. The third part involves leveraging 2D annotation information to assist the training of the 3D detection model, enabling good detection performance even in the absence of 3D annotation information.}
    \label{cover_figure}
    \vspace{-20pt}
\end{figure}



\begin{figure*}[t]
    \setlength{\abovecaptionskip}{0pt}
    \setlength{\belowcaptionskip}{0pt}
    \centering
    \includegraphics[width=1.0\linewidth]{secs/pictures/5_datasets_final.png}
    \captionsetup{font={footnotesize}}
    \captionsetup{justification=justified} % 设置 caption 文字两端对齐
    \caption{Visualizations of the detection results of our method on five different datasets: BDD100K, Cityscapes, KITTI, nuScenes, and ONCE.}
    \label{five_dataset}
    \vspace{-15pt}
\end{figure*}


Despite the progress made, the implementation of monocular 3D object detection still faces significant obstacles, with data being a primary issue \cite{peng2022lidar}. When attempting to deploy a 3D detection model on a robot equipped with a single camera in a new setting, acquiring 3D data labeled with LiDAR points poses a challenge, and refining the model with data collected from the robot is not feasible. As such, it is crucial to rely on the pretrained model's ability to generalize effectively with minimal zero-shot fine-tuning.


Given these obstacles, we propose strategies aimed at enhancing the implementation of monocular 3D detection models by making efficient use of available data. Initially, we investigate the complexities of training vision-based 3D detection models using a diverse range of public 3D datasets with different camera settings. Through this process, we develop an output representation for the monocular 3D detection model that is unaffected by variations in camera settings and simultaneously create a framework for training models on datasets with diverse annotations. This method has the potential to significantly increase the scalability of models for individual researchers and developers.

Following this, we propose an approach for training 3D models using 2D labels. Various existing techniques, such as MonoFlex\cite{MonoFlex}, annotate objects on the heatmap based on the projection of the 3D center onto the image rather than the center of 2D bounding boxes. We develop a training methodology that allows these models to be fine-tuned using 2D labels. This strategy enables us to refine existing models using more cost-effective 2D-labeled data collected from on-site robots, facilitating the transfer of 3D knowledge from public 3D datasets to the target environment. In this paper, we will present experiments conducted to fine-tune a pre-trained model using KITTI 2D data and Cityscapes 2D data as a demonstration of the potential effectiveness of our proposed approach.

% Moreover, by integrating the two proposed methods, we can significantly expand our monocular 3D detection models by training them on a mix of multiple public 3D/2D datasets. This dramatically enlarges the data available during the training phase, thereby significantly enhancing the generalization ability of the resulting model. 
% We pre-train a model on a combined set of KITTI, nuScenes, ONCE, Cityscapes, and BDD100K datasets and then fine-tune it on the target dataset using only 2D labels. We subsequently test the model's generalization ability on the target dataset. Fig. \ref{five_dataset} visualizes the detection performance of our algorithm on five well-known datasets.
Furthermore, through the integration of the two aforementioned methods, we can greatly enhance the scope of our monocular 3D detection models by training them on a combination of diverse public 3D/2D datasets. This approach significantly increases the volume of data utilized during training, leading to a notable improvement in the model's generalization capabilities.
We commence by pre-training a model on a merged collection of KITTI, nuScenes, ONCE, Cityscapes, and BDD100K datasets, followed by fine-tuning it on the target dataset using solely 2D labels. Subsequently, we evaluate the model's ability to generalize on the target dataset. 
% The performance of our algorithm on the five well-known datasets is depicted in Fig. \ref{five_dataset}.
Our algorithm's qualitative results on the five well-known datasets are depicted in the Fig. \ref{five_dataset}.


% The contributions of this work can be summarized as:
Our main contributions are as follows:

\begin{itemize}
\item A robust output representation for models like MonoFlex \cite{MonoFlex} was developed to accommodate different camera intrinsic parameter settings lays the foundation for training models on diverse datasets.
% \item Development of strategies to train or fine-tune 3D vision models on a blend of 3D/2D datasets.
\item We proposed a novel method for training and fine-tuning monocular 3D detection models on mixed 2D and 3D datasets. Enhanced the model's generalization performance and reduced the dependence on costly 3D labels.
% \item Extensive experiments were conducted on a combined set of KITTI, nuScenes, ONCE, Cityscapes and BDD100K datasets to assess the efficacy of our proposed methods.
\item Comprehensive experiments were conducted on the joint dataset comprising KITTI, nuScenes, ONCE, Cityscapes, and BDD100K. The results of the experiments demonstrate the effectiveness of our method. Compared to zero-shot settings, our approach achieved a significant performance improvement.
\end{itemize}

% \footnotetext{The results obtained from the unofficial implementations can be found at https://github.com/Owen-Liuyuxuan/mono3D .}



==> secs/sec-1-related-works.tex <==

\section{Related Works}
\label{section:Relate}

\subsection{Monocular 3D Object Detection}

% Recent developments in monocular 3D detection can be broadly categorized into two methodologies: bird-eye-view (BEV) methods and perspective-view (PV) methods.

% \textbf{Bird-Eye-View Methods:} These methods focus on conducting monocular 3D detection directly within 3D spaces, which simplifies the design of output representation. However, the main challenges arise in the transformation between perspective-view images and features in 3D coordinates. Pseudo-LiDAR represents a series of works that reconstruct 3D RGB-point clouds from monocular depth prediction models, subsequently applying LiDAR-based 3D object detectors to the reconstructed point cloud \cite{Weng2019Plidar,Vianney2019RefinedMPL,Ma2019AM3D,Ku2019MonoPSR}. Another approach directly performs differentiable feature transformation, constructing 3D features from image features, enabling end-to-end training of 3D detection in 3D spaces \cite{Cody2021CaDDN}. These methods often delegate the scale-ambiguity problem to depth prediction sub-networks or attention modules. However, network inferencing in the BEV space heavily relies on 3D labels from LiDAR or direct supervision from LiDAR data, making it challenging to utilize existing 2D datasets or inexpensive 2D labeling tools. Consequently, researchers with limited access to 3D labeled data may encounter difficulties when deploying or fine-tuning networks in new environments.

\textbf{Bird-Eye-View Methods:} These techniques focus on performing monocular 3D detection directly in 3D spaces, simplifying the output representation design. However, the main difficulties lie in converting perspective-view images to 3D coordinates features. 
% Pseudo-LiDAR encompasses a series of studies that reconstruct 3D RGB-point clouds from monocular depth prediction models, then applying LiDAR-based 3D object detectors to the reconstructed point cloud \cite{Weng2019Plidar,Vianney2019RefinedMPL,Ma2019AM3D,Ku2019MonoPSR}. 
In \cite{Weng2019Plidar,Vianney2019RefinedMPL,Ma2019AM3D,Ku2019MonoPSR}, researchers first predict depth information from monocular images, and then perform 3D object detection based on the predicted depth information.
Another method directly conducts differentiable feature transformation, creating 3D features from image features, enabling end-to-end training of 3D detection in 3D spaces \cite{Cody2021CaDDN}. These methods often address the scale-ambiguity issue through depth prediction sub-networks or attention modules. However, inference speed in the BEV space heavily depends on 3D labels from LiDAR or direct supervision from LiDAR data, making it difficult to leverage existing 2D datasets or cost-effective 2D labeling tools. As a result, researchers lacking access to 3D labeled data may face challenges when deploying or fine-tuning networks in new environments.

\textbf{Perspective-View Methods:} These methods perform monocular 3D detection directly in the original perspective view, which is more intuitive. Many single-stage monocular 3D object detection methods are built upon existing 2D object detection frameworks. The main challenge here lies in designing robust and accurate encoding/decoding methods to bridge 3D predictions and dense perspective view features. Various techniques have been proposed, such as SS3D \cite{Jorgensen2019SS3D}, which adds additional 3D regression parameters; ShiftRCNN \cite{Li2019ShiftRCNN}, which introduces an optimization scheme. Other works like M3DRPN \cite{Brazil2019M3DRPN}, D4LCN \cite{Ding2019D4LCN}, and YoloMono3D \cite{Liu2021YOLOStereo3D} use statistical priors in anchors to improve the accuracy of 3D regression. Additionally, SMOKE \cite{liu2020SMOKE}, RTM3D \cite{Li2020RTM3DRM}, Monopair \cite{Chen2020MonoPair}, and KM3D \cite{KM3D2020Li} leverage heatmap-based keypoint predictions, combined with anchor-free object detection frameworks like CenterNet \cite{zhou2019objects}.

Despite impressive progress in monocular 3D detection, most research still focuses on training within a single homogeneous dataset, leading to overfitting and poor generalization of models in specific camera settings. In this study, we propose a more robust output representation based on MonoFlex \cite{MonoFlex}, enabling the network to be trained on different datasets. We also introduce a training strategy for performing 3D object detection on 2D datasets, enhancing the model's generalization and reducing the annotation cost for 3D object detection.

\subsection{Weakly Supervised 3D Object Detection}
% For the 3D object detection task, annotating 3D labels is costly, prompting some studies to explore simpler annotations for training.
The weakly-supervised approach is also one of the methods aimed at reducing dependency on annotated data.
Autolabels \cite{zakharov2020autolabeling} present an automatic annotation pipeline to recover
9D cuboids and 3D shapes from pre-trained off-the-shelf 2D
detectors and sparse LIDAR data.
WS3D \cite{qin2020weakly} introduced a weakly supervised approach for 3D LiDAR object detection in two stages. Initially, cylindrical object proposals are generated by manual annotations in the bird’s eye-view. Subsequently, the network refines these proposals using a small set of precisely labeled object instances to produce the final 3D object bounding boxes. 
% VS3D \cite{qin2020weakly} trained on point cloud data to generate 3D proposals and utilized a 2D classification network to classify them. 
WeakM3D \cite{peng2022weakm3d} first detected objects in images and combined them with 3D point cloud data to obtain object-LiDAR-points. Furthermore, it proposed a method to estimate object orientation $\theta$ by determining the orientation of each point pair in the object-LiDAR-points. 
% In contrast, our approach not only operates without relying on 3D point cloud data but also achieves results comparable to some fully supervised methods.
WeakMono3D \cite{tao2023weakly} introduce a new labeling
method called 2D direction label, replacing the 3D rotation
label in point clouds data and a direction consistency loss
based on the new labels. 
% While this method still requires only 2D annotations, it introduces the need for paired image inputs to generate supervision, thereby increasing computational complexity.
Compared to the aforementioned weakly supervised methods, our approach does not require point clouds assistance, which reduces the complexity of sensors. It also does not rely on multi-view images, avoiding errors in the spatial position of objects caused by imprecise poses between multi-view images.



% \subsection{Task Incremental Learning}

% Task incremental learning represents a specific scenario within incremental learning where models are sequentially trained to recognize new classes across different training phases \cite{riemannian2018IL}. This means that the models are exposed to datasets with varying sets of annotations, particularly when employing a joint set of data labeled with different types. This approach fosters adaptability and flexibility, allowing the model to evolve and accommodate new information without losing its proficiency in previously learned tasks. It represents a significant step towards creating more dynamic and responsive learning systems, capable of adapting to the ever-changing landscape of data and information. Most of the research are focused on Softmax-based multi-class classification \cite{yun2021defense} where activations from different classes all have impacts on each output.
% In this paper, we re-formulate the categorical masking strategy in the setting of joint-dataset training under sigmoid-based classification, allowing more flexible dataset usage. 




==> secs/sec-2-methods.tex <==
\section{Methods}
\label{sec:methods}

\begin{figure*}[]
    \setlength{\abovecaptionskip}{0pt}
    \setlength{\belowcaptionskip}{0pt}
    \centering
    \includegraphics[width=1.0\textwidth]{secs/pictures/framework229.png}
    \captionsetup{font={footnotesize}}
    \captionsetup{justification=justified} % 设置 caption 文字两端对齐
    \caption{This figure illustrates the training process of our proposed method. It shows how the pre-trained model's inference, combined with the 2D annotations from the dataset, facilitates the training of a 3D detection model on datasets that lack 3D training labels.}
    \label{training}
    \vspace{-10pt}
\end{figure*}

% \subsection{Generalizable MonoFlex Detection Baseline}
\subsection{Camera Aware Monoflex Detection Baseline}
Monocular 3D object detection involves estimating the 3D location center $(x, y, z)$, dimensions $(w, h, l)$ and planar orientation $\theta$ of objects of interest with a single image. Since most SOTA detectors perform prediction in the camera's front-view, we generally predict the projection of the object center on the image plane $(c_x, c_y)$ instead of the 3D position $(x, y)$. The orientation $\theta$ is further replaced with the observation angle
\begin{equation}
    \alpha = \theta - \text{arctan}(\frac{x}{z}),
\end{equation}
% $\alpha = \theta - \text{arctan}(\frac{x}{z})$,
which better conforms with the visual appearance of the object \cite{MonoFlex, Brazil2019M3DRPN}.

% \textbf{GAC} \cite{liu2021GAC} is an anchor-based 3D detection method that produces SOTA performance on the KITTI dataset. It first extracts feature maps from the input images with a ResNet backbone \cite{He2015Resnet}. Then a ground-aware convolution head is applied to produce dense predictions of objects. As an anchor-based algorithm, GAC predicts the offset of the ground truth object from the predefined anchors $(\delta c_x, \delta c_y, \delta z, \delta w, \delta h, \delta l, \delta \alpha)$ based on the 3D statistics collected within the training set. The regression branch is trained using SmoothL1 Loss, while the classification branch is trained with a setup similar to one-stage anchor-based 2D object detectors.

 MonoFlex \cite{MonoFlex} is an anchor-free method.
% that ranks first among all the published monocular 3D detectors to date. 
It extracts feature maps from the input images with a DLA \cite{DLA2018Yu} backbone, similar to CenterNet\cite{zhou2019objects} and KM3D \cite{KM3D2020Li}. As an anchor-free algorithm, MonoFlex predicts the center positions of target objects with a heat map.
Monoflex primarily consists of the following components: 2D detection, dimension estimation, orientation estimation, keypoint estimation and depth estimation ensemble.
% For 
% It also directly predicts the relative coordinates between the keypoints and the center points $\{\delta_{ki} = k_i - x_r, i=1...8 \}$. 
% The depth prediction $z$ is simultaneously estimated from both geometry and direct prediction, and we adaptively ensemble these predictions to obtain the final result.
The depth prediction $z$ is simultaneously estimated from both geometry and direct prediction, and these predictions are adaptively ensembled to obtain the final result.

% Both anchor-based and anchor-free detectors rely on a high-quality backbone network to achieve good performance. According to the experiments conducted for MonoFlex and YOLOMono3D\cite{Liu2021YOLOStereo3D}, changing different backbone networks could significantly influence the final performance. In this paper, we aim to investigate the effect of Transformer backbones in both the anchor-based and anchor-free settings. 
Since we aim to perform joint training on diverse datasets, where data collection involves different cameras with distinct camera settings, our method needs to overcome the challenges posed by varying camera parameters in order to facilitate effective knowledge transfer across these datasets. Given that MonoFlex exhibits insensitivity to camera parameters, we build upon MonoFlex as the foundation of our approach.

% Overall, our approach is quite similar to monoflex, with the main difference being that our method has modifications in the depth prediction component, taking camera parameters into account. Specifically, in the original monoflex paper, the direct regression part of depth prediction assumes an absolute depth of 
Overall, our approach is similar to MonoFlex, with the main difference being that our method has modifications in the depth prediction component, which takes camera parameters into account. Specifically, in the original MonoFlex paper, the direct regression part of depth prediction assumes an absolute depth of
\begin{equation}
    z_{r} = \frac{1}{\sigma(z_{o})} - 1,
\end{equation}
where $z_{o}$ is the unlimited network output following \cite{Chen2020MonoPair, zhou2019objects} and 
\begin{equation}
\sigma(x) = \frac{1}{1 + e^{-x}}.
\end{equation}
While in our method, we have improved it by taking camera's parameters into account as follows:
\begin{equation}
    z_{r} = (\frac{1}{\sigma(z_{o})} - 1) \times \frac{f_{x}}{f_{x0}} .
\end{equation}
where $f_{x}$ is epresents the focal length of the camera used in the training dataset, while $f_{x0}$ is a hyperparameter, we set its value to 500 in our experiments.

% \subsection{Camera Aware Monoflex 3D Detection}


\subsection{Selective Training for Joint 3D Dataset Training}
\label{sec:why-base-vtr-failed}
During dataset training, some parts of the dataset are incompletely annotated. For instance, in the case of KITTI, certain categories like ``Tram'' are not labeled. However, it is not appropriate to treat the data from KITTI as negative samples for the ``Tram'' category. Therefore, each data point, in addition to its own annotations, is associated with the categories labeled in the respective dataset. This association provides supervision for the network's classification output and is applied only to the categories with annotations. 
Specifically, for different 3D datasets with varying labeled categories, each data frame stores the categories currently labeled in the dataset. When calculating the loss, we do not penalize (suppress) the detection predictions for unannotated categories.
In summary, this approach effectively handles the issue of incomplete annotations during dataset training. It ensures that only annotated categories influence the model's training, and unannotated categories do not lead to erroneous model behavior. The training procedure is shown in Fig. \ref{training}.


% \subsection{Regulating 2D Labels for 2D Datasets }
\subsection{Regulating 2D Labels of 2D Datasets for Pseudo 3D training}
In the Monoflex method, the center of the heatmap is determined by projecting the 3D center. For data with only 2D annotations, we have no direct means of generating supervision signals for the object's 3D center. 
Therefore, we need to find a way to generate 3D detection supervision information from 2D labels. We propose a novel method to train 3D detection algorithms solely relying on 2D detection labels. Specifically, we start by feeding data with only 2D annotations into a pre-trained 3D detection model and set a very low score threshold to enable the model to produce multiple detection results (including both 2D and 3D detection results). This step may include some erroneous or inaccurate detections.
Next, we use the 2D training labels from the new dataset to match them with the 2D detection results obtained in the previous step, filtering out erroneous or inaccurate detections to obtain pseudo 3D training labels. Finally, we reconstruct the ground truth heatmap and 2D detection map (as shown in Fig. \ref{label_update}), and ultimately, we calculate the loss between the model predictions and the pseudo 3D labels only on the heatmap and 2D detection map.
The method of training a monocular 3D model using 2D annotated data is illustrated in Algorithm \ref{alg:post}, we refer to it as \textit{Pseudo 3D Training with 2D Labels}.
\input{secs/alg_p2D}

% \subsubsection{Self-Attention-Based Head}

% \subsubsection{Geometric-aware Positional Embedding}

% \begin{figure}[t]
%     \setlength{\abovecaptionskip}{0pt}
%     \setlength{\belowcaptionskip}{0pt}
%     \centering
%     \includegraphics[width=1.0\linewidth]{secs/pictures/spider_plot.png}
%     \captionsetup{font={footnotesize}}
%     \captionsetup{justification=justified} % 设置 caption 文字两端对齐
%     \caption{The comparison between our method and zero-shot on the Cityscapes dataset shows that our method outperforms zero-shot in all the evaluation metrics.}
%     \label{spider_plot}
% \end{figure}



\begin{figure*}[]
    \setlength{\abovecaptionskip}{0pt}
    \setlength{\belowcaptionskip}{0pt}
    \centering
    \includegraphics[width=1.0\linewidth]{secs/pictures/label_update229b.png}
    \captionsetup{font={footnotesize}}
    \captionsetup{justification=justified} % 设置 caption 文字两端对齐
    \caption{The figure depicts the training label update process. In the left image, the pre-trained 3D detection model's predictions on new data are shown, which may include some erroneous detections, as indicated by the green boxes. The middle image illustrates the process of identifying and filtering out these erroneous detections, marking them in gray based on the matching results. The right image represents the reconstruction of the ground truth heatmap using the pseudo 3D labels.}
    \label{label_update}
\end{figure*}

==> secs/sec-3-experiments.tex <==

\section{Experiments}
\label{section:Experiments}

\input{secs/tabel_nusc_kitti}
\input{secs/table_cityscapes}
\input{secs/table_weakly_supervised}


\subsection{Datasets Reviews}

We evaluate the proposed networks on the KITTI 3D object detection benchmark \cite{Geiger2012KITTI} and Cityscapes dataset \cite{gahlert2020cityscapes}. The KITTI dataset consists of 7,481  training frames and 7,518 test frames. Chen \textit{et al.} \cite{Chen2015kittisplit} split the training set into 3,712 training frames and 3,769 validation frames. The Cityscapes dataset contains 5000 images split into 2975 images for training, 500 images for validation, and 1525 images for testing. 

% All the testing and validation results, are evaluated with 40 recall positions ($AP_{40}$), following Simonelli \textit{et al.} \cite{Simonelli2019MonoDIS} and the KITTI team. Such a protocol is considered to be more stable than the $AP_{11}$ proposed in the Pascal VOC benchmark \cite{Everingham10pascal}.

% For the anchor-based method SwinMono3D, we apply a pretrained Swin-B as the backbone, which is comparable to the ResNet-101 backbone used in the GAC model. The proposed model is trained for 30 epochs on the training frames, following the training settings of GAC \cite{liu2021GAC} and YOLOMono3D \cite{Liu2021YOLOStereo3D}.

% For the anchor-free method SwinFlex, we use a pretrained Swin-T as the backbone to replace the DLA-34 backbone in MonoFlex. The proposed model is trained for 200 epochs on the training frames, following the original settings of MonoFlex \cite{MonoFlex} and RTM3D \cite{Li2020RTM3DRM}.

\subsection{Evaluation Metrics}
\subsubsection{KITTI 3D}
All the testing and validation results, are evaluated with 40 recall positions ($AP_{40}$), following Simonelli \textit{et al.} \cite{Simonelli2019MonoDIS} and the KITTI team. Such a protocol is considered to be more stable than the $AP_{11}$ proposed in the Pascal VOC benchmark \cite{Everingham10pascal}.
\subsubsection{Cityscapes 3D}
Following \cite{gahlert2020cityscapes}, we use these five metrics: 2D Average Precision $(AP)$, Center Distance $(BEVCD)$, Yaw Similarity $(YawSim)$, Pitch-Roll Similarity $(PRSim)$, Size Similarity $(SizeSim)$ and Detection Score $(DS)$ to evaluate the performance on Cityscapes 3D dataset. Among them, $DS$ is a combination of the first five metrics and computed as:
\begin{footnotesize}
\begin{equation}
 DS = AP \times \frac{BEVCD+YawSim+PRSim+SizeSim}{4}. 
\end{equation}
\end{footnotesize}
For details, please refer to the paper \cite{gahlert2020cityscapes}.

\subsection{Experiment Setup}
To demonstrate the effectiveness of our method, we conducted extensive experiments on the KITTI and Cityscapes datasets. When testing on the KITTI dataset, we designed our experiments as follows:

\begin{itemize}
    % \item Testing on KITTI Dataset:
    % \begin{itemize}
        \item We initially pre-trained our model on four datasets: BDD100K, nuScenes, ONCE, and Cityscapes.
        \item With the pre-trained model, we evaluated its zero-shot detection performance on the KITTI dataset.
        \item Subsequently, we fine-tuned the model using our method, which involves training a 3D detection model using 2D training labels from KITTI.
        \item Finally, we obtained detection results on the KITTI dataset based on our method.
    % \end{itemize}
    % \item Testing on Cityscapes Dataset:
    % \begin{itemize}
    %     \item Similar to the KITTI experiment, we pre-trained our model on four datasets: BDD100K, nuScenes, ONCE, and KITTI.
    %     \item Using the pre-trained model, we assessed its zero-shot detection performance on the Cityscapes dataset.
    %     \item Following that, we employed our method to adjust the model, which entails training a 3D detection model using 2D training labels from KITTI.
    %     \item Ultimately, we obtained detection results on the Cityscapes dataset based on our method.
    % \end{itemize}
    
\end{itemize}

When testing on the Cityscapes dataset, we followed the same experimental setup on the KITTI dataset.

% 1. **Tes;r method.

% In summary, our experimental setup involves pre-training our model on multiple datasets and then evaluating its zero-shot detection capabilities on a target dataset (KITTI or Cityscapes). Subsequently, we fine-tune the model using our proposed method, which leverages 2D training labels from the KITTI dataset to train the 3D detection model. This approach allows us to achieve improved detection results on both the KITTI and Cityscapes datasets.


\subsection{Experiment Results and Comparison}
The quantitative results of the ``Car'', ``Pedestrain'' and ``Cyclist''  category on KITTI dataset are reported in Table~\ref{tab:test_results}, while quantitative results of ``Car'', ``Truck'' and ``Bicycle'' category on Cityscapes dataset are shown in Table~\ref{tab:test_results_city_car}, Table~\ref{tab:test_results_city_truck}, and Table~\ref{tab:test_results_city_Bicycle} respectively.

\begin{figure}[]
    \setlength{\abovecaptionskip}{0pt}
    \setlength{\belowcaptionskip}{0pt}
    \centering
    \includegraphics[width=1.0\linewidth]{secs/pictures/concat_image_5.png}
    \captionsetup{font={footnotesize}}
    \captionsetup{justification=justified} % 设置 caption 文字两端对齐
    \caption{The qualitative results on the Cityscapes dataset. The leftmost column contains the original images, the middle column displays the zero-shot results, and the rightmost column shows the results obtained using our method. The pink boxes represent 2D detection results.}
    \label{vis_compare}
    \vspace{-10pt}
\end{figure}

% We also utilized radar charts to visualize the performance on the Cityscapes dataset, as depicted in Fig. \ref{spider_plot}. 



From Table~\ref{tab:test_results}, we can observe that our method has achieved significant improvements in both 3D and 2D detection tasks compared to zero-shot learning. 
% Specifically, for the 3D detection task, our method has shown an improvement in $AP_{3D}$ for the ``Car'' category in the easy, moderate, and hard difficulty levels by 16.42\%, 4.27\%, and 0.20\%, respectively. 
% Specifically, for the 3D detection task, we achieved $AP_{3D}$ of 48.99, 33.29, 28.41 and $AP_{BEV}$ of 56.87, 39.17, 33.79, in terms of the Easy, Moderate and Hard categories.
% In the ``Pedestrian'' and ``Cyclist'' classes, at the Easy, Moderate and Hard difficulty levels, we achieved $AP_{3D}$ scores of 14.09, 12.95 and 10.79 for ``Pedestrian'', and 1.57, 0.84 and 0.81 for ``Cyclist'', respectively. The $AP_{BEV}$ scores were 56.87, 39.17 and 33.79 for ``Pedestrian'', and 1.86, 1.06 and 1.01 for ``Cyclist'', respectively.
Specifically, for the 3D detection task, our method has shown an improvement in $AP_{3D}$/$AP_{BEV}$ for the ``Car'' category in the Easy, Moderate, and Hard difficulty levels by $18.55/18.67$, $10.10/10.32$ and $8.20/8.37$, respectively. 
In the ``Pedestrian'' category, we achieved a progress in $AP_{3D}$/$AP_{BEV}$ in the Easy, Moderate, and Hard difficulty levels by $7.29/7.90$, $7.13/7.28$ and $5.72/5.94$, respectively.
And for the ``Cyclist'' category, we improved the $AP_{3D}$/$AP_{BEV}$ by $0.93/0.57$, $0.47/0.24$ and $0.46/0.48$ in Easy, Moderate and Hard level, respectively. 
For the ``Cyclist'' class, although there is not a significant increase in the number of 3D detection points, the improvement in AP3D/APBEV across three different difficulty levels ranges from 29.27\% to 145.32\%. Therefore, the improvement from our method is significant.
In summary, the experimental results demonstrate the effectiveness of our method on the KITTI dataset.
% These improvements are significant, demonstrating the effectiveness of our approach.
% In the ``Pedestrian'' category, the AP improvements are even more substantial, with increases of 50.7\%, 32.73\%, and 35.34\% for the easy, moderate, and hard difficulty levels, respectively.
% The improvements in $AP_{2D}$ for the ``Car'' category in the easy, moderate, and hard difficulty levels by 5.54\%, 11.25\%, and 12.39\%, respectively, as well as the AP enhancements of 5.69\%, 6.83\%, and 8.80\% in the ``Pedestrian'' category across the same difficulty levels for the 2D detection task. These improvements in 2D detection performance are easily comprehensible because we trained the algorithm comprehensively on the new dataset using 2D training labels.

Table~\ref{tab:test_results_city_car}, Table~\ref{tab:test_results_city_truck} and Table~\ref{tab:test_results_city_Bicycle} present the detection results for the ``Car'', ``Truck'' and ``Bicycle'' categories on the Cityscapes dataset. Quantitative results indicate that our method, when compared to the zero-shot approach, has shown significant improvements in various metrics, except for the PRSim metric (as we only focused on the yaw angle, considering pitch and roll angles to be 0). Specifically, in the ``Car'' category, we observed an increase of $25.05$ in AP, a $0.69$ improvement in BEVCD, a $2.15$ improvement in YamSim, a $6.18$ improvement in SizeSim, and a remarkable $24.02$ enhancement in DS. 
In the ``Truck'' category, AP, BEVCD, YawSim, SizeSim, and DS have improved by $13.71$, $0.85$, $0.06$, $12.50$, and $13.12$, respectively.
And for the ``Bicycle'' class,AP, BEVCD, YawSim, SizeSim, and DS have improved by $2.77$, $3.50$, $5.21$, $11.74$, and $2.35$, respectively.
% From these experimental results, we can also observe that our method demonstrates a more significant improvement in detection performance for categories with fewer instances in the dataset. This is due to the fact that the model has less knowledge about categories with fewer instances, leading to weaker generalization on new datasets compared to categories with more instances. 
% From these experimental results, we can observe that after pseudo 3D learning using 2D labels on the new dataset, we achieved a substantial improvement in detection performance.
From the above experimental results, it can be seen that our method has also achieved significant performance improvement on the Cityscapes dataset.
% Our proposed method exhibits significant improvements over zero-shot learning across five key metrics: AP (Average Precision), BEVCD (Bird's Eye View Center Distance), YawSim (Yaw Similarity), SizeSim (Size Similarity), and DS (Detection
% Score). Fig. \ref{vis_compare} illustrates the qualitative results on the Cityscapes dataset.
Fig. \ref{vis_compare} provides a visual comparison between our method and the zero-shot approach. It can be observed that our method exhibits significantly improved detection capability compared to the zero-shot approach.

Table~\ref{tab:weakly_supervised} illustrates the comparison between our method and several weakly-supervised methods on the ``Car'' class in the KITTI dataset. It is apparent that overall, our method falls short of the latest state-of-the-art algorithm, WeakMono3D \cite{tao2023weakly}. However, it outperforms other weakly-supervised algorithms. It is worth mentioning that our approach relies solely on easily accessible 2D annotations, without requiring any 3D annotation information or additional sensor data such as point clouds or multi-view images for assistance.

% Most of the annotated objects in the KITTI dataset are the Car type, and the proposed anchor-based SwinMono3D and anchor-free SwinFlex outperform existing methods, beating their CNN-based counterparts. We further note that ours are the first models that fully consist of perceptrons and self-attention layers, while all existing methods are based on convolutional networks.

% SwinMono3D and SwinFlex perform much better than existing works on Pedestrian prediction, which is mainly due to the improved information exchange between all foreground pixels. The anchor-based SwinMono3D does not perform well on the Cyclist type, mainly because anchor-based methods rely on statistics in the training set, and there are too few Cyclists in the training set to learn from. Such a problem can also be observed in D4LCN \cite{Ding2019D4LCN} and M3D-RPN ~\cite{Brazil2019M3DRPN}.

% We present qualitative results of the anchor-based SwinMono3D in Figure~\ref{spider_plot}. The SwinMono3D shown here is trained on Chen's training sub-split. The proposed model can detect and localize most of the Cars well, like other SOTA methods. It can also accurately detect Pedestrians, which could be truncated or have a similar texture to the background. From the examples on the top-left, we can find that far-away objects are still difficult to detect, and there could be orientation errors in the localization. 

% We provide an ablation study of the model in the following section.

% \section{Zeroshot Generalization and Discussion}
% \label{section:AblationStudy}

% In this section, we analyze the performance of the proposed model and discuss the effectiveness of our proposed design choices. These experiments are conducted on Chen's split of the KITTI dataset.


% \subsection{Swin Backbone and Attention Head}

% In Section~\ref{sec:why-base-vtr-failed}, we presented possible reasons why the basic ViT model failed. We also explained the initial motivation for choosing the Swin Transformer as the backbone. Here, we further provide numerical results on the performance of the Swin backbone and the attention head in Table.

% From the ablation experiments, we discover that it is the combination of the Swin backbone and the attention-based head that most significantly boosts the performance of the proposed model. The attention-head is a significant performance booster in the original CNN-based model because it allows global information exchange. While the Swin backbone suffers from a relatively small receptive field, the attention head fully exploits the potential of the Swin backbone, and this combination achieves the best performance in the experiment.


% % \input{secs/table_campus}

% % \input{secs/ablation_ped_cyc.tex}
% \subsection{Geometric-aware Positional Embedding}

% GEM is proposed to inject both positional information and geometric information into the model. We compare GEM with two other popular embedding methods commonly used in ViTs: 1D embedding \cite{dosovitskiy2020vit}, which is a learnable constant parameter with the same shape as the input feature map, and Sine-Cosine embedding is also commonly used in visual Transformers \cite{Ashish2017Attention}, where the absolute position of each pixel in the image is encoded with sinusoidal functions. 

% From the results presented in Table, we discover that the proposed GEM embedding can improve upon the 3D detection results by a noticeable margin. We further note that the choice of positional embedding does not have a statistically significant impact on the 2D detection results, so the major improvement is in the accuracy of 3D reasoning.

% \subsection{Self-Attention Map Visualization}

% The self-attention layer is also renowned for its explainability. By visualizing the attention map of the self-attention layer, we can understand the behavior of the network to an extent. 


% We visualize the attention map produced by SwinMono3D on an image from the validation set in Figure~\ref{fig:attention_showing}. The detection results are presented in the top-left image, where we select three detected objects and visualize the attention map of their center pixels. 

% For a clearly detectable pedestrian or a standalone car in this image, the self-attention layer will concentrate on the pixels around the center object pixel, as shown in the two attention maps at the bottom of the figure. However, for a pedestrian that is more difficult to detect, the network will try to fuse information from other front-ground objects and distinguish the pedestrian from the background, as demonstrated by the attention map on the top-right corner of the figure.

% As a result, the network implicitly extracts information from other foreground objects to help in the detection of harder objects. It could partially explain the improvement presented by the proposed method in Pedestrian and Cyclist detection in the KITTI dataset, where the number of labeled instances is rather small.






==> secs/sec-4-conclusion.tex <==

\section{Conclusion}
\label{section:Conclusion}

% For supervised learning, training labels are crucial, and manual data annotation is a time-consuming and costly process. This is especially true for monocular 3D detection tasks, where annotating training data often requires the coordination of LiDAR and camera data, further increasing the complexity and cost of data labeling. In contrast, general 2D detection labeling is comparatively easier and can even be semi-automated using pre-trained models. Therefore, we aim to improve monocular 3D detection performance on new datasets relying solely on 2D labels.
% In this paper, we first conducted research on models like MonoFlex and devised strategies that are robust to changes in camera intrinsics. These strategies enable the models to be trained on different datasets. Additionally, we designed a learning strategy that allows monocular 3D detection models to learn 3D detection tasks relying solely on 2D labels, even in datasets that provide only 2D training labels. Finally, we conducted extensive experiments on a combination of datasets, including KITTI, nuScenes, cityscapes, and others. The experimental results demonstrated the effectiveness of our approach.
% In supervised learning, training labels are essential, and manual data annotation can be a time-consuming and costly process. This is especially true for monocular 3D detection tasks, wherein annotating training data often necessitates the coordination of LiDAR and camera data, further increasing the complexity and expense of data labeling. In contrast, general 2D detection labeling is comparatively simpler and can even be semi-automated using pre-trained models. Consequently, our goal is to enhance monocular 3D detection performance on new datasets that rely solely on 2D labels.
In this paper, we initially conducted research on models such as MonoFlex \cite{MonoFlex} and developed strategies that are resilient to changes in camera intrinsics. These strategies allow the models to be trained on diverse datasets. Additionally, we designed a learning approach that enables monocular 3D detection models to acquire 3D detection knowledge based solely on 2D labels, even in datasets that only provide 2D training labels. Lastly, we carried out extensive experiments on a combination of datasets, including KITTI, nuScenes, Cityscapes, and others. The experimental results demonstrated the efficacy of our approach.
% Specifically, on the KITTI dataset, our method improved 3D detection performance by up to 16.42\% compared to zero-shot learning in the 'Car' category. In the 'Pedestrian' category, the improvement was even more significant, with an increase of up to 50.7\%. On the Cityscapes dataset, our method achieved a detection score increase of 17.84\% in the 'Car' category and a remarkable 115.91\% increase in the 'Truck' category. This represents a substantial improvement in performance.
% Despite its success, our work does have some limitations. Firstly, our method is currently applicable only to models that are insensitive to camera parameters, such as MonoFlex. For models where the influence of camera parameters cannot be disregarded, further improvements to our method are necessary.
% Furthermore, when dealing with new categories on a novel dataset, the absence of relevant supervision from previous datasets may lead to suboptimal detection performance for these new categories. Addressing this limitation also requires ongoing optimization and enhancement of our approach.
Despite its success, our work does have limitations. First, our method is currently applicable only to algorithms that are insensitive to camera parameters, such as MonoFlex. For models where the influence of camera parameters cannot be disregarded.
% further refinements to our method are necessary.
Moreover, when encountering new categories in a novel dataset, the lack of relevant supervision from previous datasets may result in suboptimal detection performance for these new categories. 
% Overcoming these limitations demands continuous optimization and improvement of our approach. 
% In future work, we will explore open-vocabulary object detection to improve the algorithm's detection performance on novel categories.
In future work, we will explore how to reduce the algorithm's sensitivity to sensor parameters to make our method more versatile. Additionally, we will investigate open-vocabulary object detection to enhance the algorithm's detection performance on new categories.

% Despite its success, our work does have certain limitations. First, our method is currently applicable only to models that are insensitive to camera parameters, such as MonoFlex. For models where the influence of camera parameters cannot be disregarded, further refinements to our method are necessary. Moreover, when encountering new categories in a novel dataset, the lack of relevant supervision from previous datasets may result in suboptimal detection performance for these new categories. Overcoming this limitation also demands continuous optimization and improvement of our approach.

==> secs/table_campus.tex <==
\begin{table}
    \centering
    \caption{2D Detection Results on Campus' Data, evaluate with $IoU_{2D} \geq 0.5$}
    \def\arraystretch{1.3}
    \begin{tabular*}{0.28\textwidth}{ |l|c|c|}
        \hline
        {\bf Methods} & {\bf Car} & {\bf Ped}   \\ \hline
        kittiMonoFlex & 55.4\% & 27.7\%  \\
        \hline
        TunedMonoFlex & 86.7\% &  81.90\%  \\
        \hline
    \end{tabular*}
    
    \label{tab:test_results_campus}
\end{table}

==> secs/table_kitti.tex <==

\begin{table*}[]
\caption{Performance of full-scale MonoDepth on KITTI360 Fisheye. We directly evaluate the error without compensating scales. The \cellcolor{red!25}{pink} columns are error metrics, the lower the better; the \cellcolor{blue!25}{blue} columns are accuracy metrics, the higher the better.}
    \label{tab:kitti_test}
    \centering
    \begin{tabular*}{0.76\textwidth}{|l|c|c|c|c|c|c|c|}
    \hline {\bf Methods} &  \cellcolor{red!25}{\bf {Abs Rel}} & \cellcolor{red!25}{Sq Rel} & \cellcolor{red!25}{ RMSE} & \cellcolor{red!25}{RMSE LOG} & \cellcolor{blue!25}{$\delta<1.25$} & \cellcolor{blue!25}{$\delta<1.25^2$} & \cellcolor{blue!25}{$\delta<1.25^3$} \\ 
    \hline
       \textbf{FSNet (all depth)}   & \textbf{0.161}  &   \textbf{0.594}  &   \textbf{2.348}  &   \textbf{0.823}  &   \textbf{0.771}  &   \textbf{0.881}  &   \textbf{0.927}  \\
       \textbf{FSNet (within 8m)}     & \textbf{0.084}  &   \textbf{0.318}  &   \textbf{0.772}  &   \textbf{0.185}  &   \textbf{0.940}  &   \textbf{0.980}  &   \textbf{0.991}  \\
      \hline
    \end{tabular*}
    
\end{table*}

\begin{table*}[]
\caption{Performance of full-scale MonoDepth on KITTI Eigen Split. For scale factor, "GT" is using LiDAR median scaling methods and "None" means we directly evaluate the error without compensating scales. "\textbf{*}" indicates methods using sequential images in test time. The \cellcolor{red!25}{pink} columns are error metrics, the lower the better; the \cellcolor{blue!25}{blue} columns are accuracy metrics, the higher the better.}
    \label{tab:kitti_test}
    \centering
    \begin{tabular*}{0.88\textwidth}{|l|c|c|c|c|c|c|c|c|}
    \hline {\bf Methods} & {\bf Scale Factor} &  \cellcolor{red!25}{Abs Rel} & \cellcolor{red!25}{Sq Rel} & \cellcolor{red!25}{\bf RMSE} & \cellcolor{red!25}{RMSE LOG} & \cellcolor{blue!25}{$\delta<1.25$} & \cellcolor{blue!25}{$\delta<1.25^2$} & \cellcolor{blue!25}{$\delta<1.25^3$} \\ 
    \hline
    MonoDepth \cite{monodepth2} & GT  &   0.116  &   0.903  &   4.863  &   0.193  &   0.877  &   0.959  &   0.981  \\
     DNet \cite{xue2020toward} &  GT &  0.113  &   0.864  &   4.812  &   0.191  &   0.877  &   0.960  &   0.981  \\
     % ManyDepth* \cite{manydepth2021temporal} & GT & 0.098 & 0.770 & 4.459 & 0.176 & 0.800 & 0.965 & 0.983 \\
    % MultiChannel (FSNet) & GT &  0.117  &   0.895  &   4.762  &   0.191  &   0.872  &   0.959  &   0.982  \\
    %  + Optical Flow (FSNet) &  GT & 0.117  &   0.881  &   4.746  &   0.191  &   0.873  &   0.959  &   0.981  \\
     \textbf{FSNet (single frame)} & GT  &   \textbf{0.113}  &   \textbf{0.857}  &   \textbf{4.623}  &   \textbf{0.189}  &   \textbf{0.876} &   \textbf{0.960}  &   \textbf{0.982}  \\
      \textbf{*FSNet (post-opt)}  & GT  & \textbf{0.111}  &   \textbf{0.829}  &   \textbf{4.393}  &   \textbf{0.185}  &   \textbf{0.883}  &   \textbf{0.961}  &   \textbf{0.983}  \\
    \hline
     DNet \cite{xue2020toward} & None &  0.118  &   0.925  &   4.918  &   0.199  &   0.862  &   0.953  &   0.979 \\
    % MultiChannel (FSNet) & None &   0.123  &   0.936  &   4.910  &   0.202  &   0.857  &   0.954  &   0.980  \\
    %+ Optical Flow (FSNet) &  None &  0.118  &   0.924  &   4.861  &   0.200  &   0.860  &   0.955  &   0.980  \\
       \textbf{FSNet (single frame)} &  None  & \textbf{0.116}  &   \textbf{0.923}  &   \textbf{4.694}  &   \textbf{0.194}  &   \textbf{0.871}  &   \textbf{0.958}  &   \textbf{0.981}  \\
       \textbf{*FSNet (post-opt)}   & None  & \textbf{0.109}  &   \textbf{0.866}  &   \textbf{4.450}  &   \textbf{0.189}  &   \textbf{0.879}  &   \textbf{0.959}  &   \textbf{0.982}  \\
      \hline
    \end{tabular*}
    
\end{table*}





==> secs/table_nusc_kitti_backup.tex <==
\begin{table*}[h!]
    \centering
    \caption{Object detection results on the KITTI validation set. For 3D metrics, cars are evaluated with $\text{IoU}_{3D} \geq 0.5$ and Pedestrians are evaluated with $\text{IoU}_{3D} \geq 0.25$; for 2D metrics, cars are evaluated with $\text{IoU}_{2D} \geq 0.7$ and Pedestrians are evaluated with $\text{IoU}_{2D} \geq 0.5$. }
    %\footnotesize
    \def\arraystretch{1.3}
    \begin{tabular*}{0.7\textwidth}{ |c|l|c|c|}
        \cline{1-4}
        {Method} &{\bf Methods} & {\bf Car Easy/Moderate/Hard} & {\bf Ped. Easy/Moderate/Hard}   \\ \cline{1-4}
        \multirow{2}{*}{$3D$} &NuscMonoFlex & 30.69\% / 23.88 \%/ 20.34 \% &  7.83\% / 6.66\% / 5.49\%  \\
        \cline{2-4}
        &TunedMonoFlex & 35.73\% / 24.90 \%/ 20.38 \% &  11.80\% / 8.84\% / 7.43\%  \\
        \cline{1-4}
        \multirow{2}{*}{$2D$} &NuscMonoFlex & 90.91\%/ 81.28\%/ 71.50\% &  59.04\%, 50.84\%, 43.76\%  \\
        \cline{2-4}
        &TunedMonoFlex & 95.95\%/ 90.42\%/ 80.36 \% &  62.40\%, 54.31\%, 47.61\%  \\
        \cline{1-4}
    \end{tabular*}
    
    \label{tab:test_results_on_cityscapes}
\end{table*}

==> secs/table_weakly_supervised.tex <==
\begin{table}[h!]
    \centering
    \caption{Comparison with weakly-supervised methods on the ``Car'' category on KITTI dataset. }
    %\footnotesize
    % \def\arraystretch{1.3}
    \renewcommand{\arraystretch}{1.2} %调行距
    \setlength\tabcolsep{3pt} %调列距
    \begin{tabular*}{0.96\textwidth}{c c c c}
        \cline{1-4}
        \multirow{2}{*}{\bf Methods} & \multicolumn{3}{c}{ $AP_{BEV}$ / $AP_{3D}$ }   \\ 
        \cline{2-4}
        % \cline{3-8}
          & {\bf Easy (\%)} & {\bf Moderate (\%)}& {\bf Hard (\%)}   \\ \cline{1-4}
         VS3D \cite{qin2020weakly} & 31.59/22.62 &  20.59/14.43 & 16.28/10.91  \\
        % \cline{2-11}
        WeakM3D \cite{peng2022weakm3d}  & 58.20/50.16 & 38.02/29.94 
                        & 30.17/23.11   \\
        Autolabels \cite{zakharov2020autolabeling}  & 50.51/38.31 & 30.97/19.90 
                        & 23.72/14.83   \\
        % \cline{1-11}
        WeakMono3D \cite{tao2023weakly}  & 54.32/\textbf{49.37}  & \textbf{42.83}/\textbf{39.01}  
                        & \textbf{40.07}/\textbf{36.34}   \\
        Ours  & \textbf{56.87}/48.99  & 39.17/33.29  
                        & 33.79/28.41      \\
        \cline{1-4}
    \end{tabular*}
    
    \label{tab:weakly_supervised}
\end{table}
